Airborne Magnetic Anomaly Navigation with Neural-Network-Augmented Online Calibration

Airborne Magnetic Anomaly Navigation (MagNav) provides a jamming-resistant and robust alternative to satellite navigation but requires the real-time compensation of the aircraft platform's large and dynamic magnetic interference. State-of-the-art solutions often rely on extensive offline calibration flights or pre-training, creating a logistical barrier to operational deployment. We present a fully adaptive MagNav architecture featuring a "cold-start" capability that identifies and compensates for the aircraft's magnetic signature entirely in-flight. The proposed method utilizes an extended Kalman filter with an augmented state vector that simultaneously estimates the aircraft's kinematic states as well as the coefficients of the physics-based Tolles-Lawson calibration model and the parameters of a Neural Network to model aircraft interferences. The Kalman filter update is mathematically equivalent to an online Natural Gradient descent, integrating superior convergence and data efficiency of state-of-the-art second-order optimization directly into the navigation filter. To enhance operational robustness, the neural network is constrained to a residual learning role, modeling only the nonlinearities uncorrected by the explainable physics-based calibration baseline. Validated on the MagNav Challenge dataset, our framework effectively bounds inertial drift using a magnetometer-only feature set. The results demonstrate navigation accuracy comparable to state-of-the-art models trained offline, without requiring prior calibration flights or dedicated maneuvers.

==> decoupling_toymodel.tex <==
\subsubsection{Decoupled Kalman Filter Architectures}
\label{sssec:decoupling}
\todo[inline, color = green]{This entire section \cref{sssec:decoupling} of decoupling for the toymodel can be taken out of this paper and presented as an individual thing (potentially testing it also on the real dataset?), focusing on decoupled architectures being benefitial for aircraft systems}

While the centralized, fully-coupled EKF provides a mathematically optimal solution by explicitly modeling the cross-correlations between navigation states and the neural network parameters, its computational demand due to the propagation of the full $n \times n$ covariance matrix $\covP$ may be prohibitive in real-world applications. For safety-critical avionics, the propagation of a large, monolithic covariance matrix presents challenges for both resource-constrained processors and the stringent certification requirements of standards like DO-178C.

Therefore, decoupled architectures represent a pragmatic engineering trade-off. By selectively simplifying or ignoring cross-covariance terms, these filters can align with \textbf{Integrated Modular Avionics (IMA)} principles, treating - in our case - navigation and calibration as separate, verifiable components. This modularity enhances computational tractability and simplifies the certification pathway, accepting a potential loss in theoretical optimality for a significant gain in the safety, modularity, and maintainability required for operational deployment.

\subsubsection*{Investigated Decoupling Strategies}

To systematically investigate the trade-off between estimation accuracy and computational complexity, four EKF configurations were implemented and evaluated:

\begin{itemize}
    \item \textbf{Level 0 (Fully Coupled):} The baseline, standard EKF which retains all cross-correlation terms within the state covariance matrix, providing the highest theoretical accuracy.

    \item \textbf{Level 1 (State/Model Decoupling):} A block-diagonal structure is enforced, decoupling the vehicle's kinematic state from the entire block of neural network parameters ($\boLambda$).

    \item \textbf{Level 2 (Layer-Wise Decoupling):} This extends the approximation by fully decoupling all parameter blocks, treating the vehicle state, each weight matrix ($\mathbf{W}^{(1)}, \mathbf{W}^{(2)}$), and each bias vector ($\mathbf{b}^{(1)}, \mathbf{b}^{(2)}$) as mutually uncorrelated.

    \item \textbf{Level 3 (Full Parameter Decoupling):} The most aggressive simplification, where the covariance submatrix for the NN parameters is forced to be purely diagonal, assuming all individual weights and biases are uncorrelated.
\end{itemize}

These levels allow for a systematic evaluation of how simplifying the cross-covariance assumptions impacts the filter's ability to learn the noise model and improve navigation accuracy.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsubsection*{Analysis of Results}

The performance of the four EKF decoupling strategies was evaluated based on the collected Monte Carlo simulation data. The analysis focuses on three key areas: the trade-off between estimation accuracy and computational runtime, the robustness and consistency of the estimators, and a comparison of the results to theoretical performance limits.

\paragraph{Overall Performance and Runtime Trade-offs}

A comprehensive overview of filter performance across all feature sets and neural network complexities is presented in Figure \ref{fig:full_performance_grid}. The results indicate that the standard, fully-coupled EKF (Level 0) is the superior configuration for this estimation problem in the framework of our implementation.

The top row of Figure \ref{fig:full_performance_grid} (a-c) illustrates the estimation accuracy as a function of neural network complexity. Across all three feature sets, the Level 0 filter consistently achieves the highest accuracy and converges with the fewest neurons (typically 8-12). The decoupled filters (Levels 1-3) demonstrate a significant performance degradation, especially with the information-rich "All Inputs" feature set, where they struggle to converge and exhibit large errors even with complex models.

The middle row (d-f) presents the average runtime. Counter-intuitively, the theoretically more complex Level 0 filter was often the fastest or among the fastest, particularly for models with low-to-moderate complexity. This phenomenon is attributed to the software environment: MATLAB's highly optimized linear algebra libraries execute the consolidated matrix operations of the Level 0 update very efficiently. In contrast, the fragmented logic of the decoupled filters, which involves numerous high-level data-slicing and reassembly operations, incurs significant interpreter overhead that negates the theoretical reduction in floating-point operations.

This conclusion is solidified by the accuracy-versus-runtime trade-off plots in the bottom row (g-i). For all three feature sets, the Level 0 results (blue dots) consistently dominate the Pareto front, occupying the optimal bottom-left region of the plot. However, this performance-centric view is incomplete for operational systems. The decision must account for the fact that these MATLAB runtimes are not representative of a compiled, real-time implementation and, more critically, that the architectural benefits of decoupling—namely simplified certification and system modularity—are often the primary drivers of the final design.

% --- FIGURE 1: 3x3 Performance Grid ---
\begin{figure}[p] 
    \centering
    \makebox[0.32\textwidth]{\textbf{All Inputs}} \hfill
    \makebox[0.32\textwidth]{\textbf{Map Val + Vel}} \hfill
    \makebox[0.32\textwidth]{\textbf{Map Val}}
    \vspace{0.2cm}
    
    % --- Row 1: Accuracy vs. Complexity ---
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/decoupling/AccuracyVsComplexity_AllInputs.png}
        \caption{Accuracy vs. Complexity}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/decoupling/AccuracyVsComplexity_MapVal_Vel.png}
        \caption{Accuracy vs. Complexity}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/decoupling/AccuracyVsComplexity_MapVal.png}
        \caption{Accuracy vs. Complexity}
    \end{subfigure}
    \vspace{0.5cm}

    % --- Row 2: Runtime vs. Complexity ---
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/decoupling/RuntimeVsComplexity_AllInputs.png}
        \caption{Runtime vs. Complexity}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/decoupling/RuntimeVsComplexity_MapVal_Vel.png}
        \caption{Runtime vs. Complexity}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/decoupling/RuntimeVsComplexity_MapVal.png}
        \caption{Runtime vs. Complexity}
    \end{subfigure}
    \vspace{0.5cm}
    
    % --- Row 3: Accuracy vs. Runtime ---
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/decoupling/AccuracyVsRuntimeTradeoff_AllInputs.png}
        \caption{Accuracy vs. Runtime}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/decoupling/AccuracyVsRuntimeTradeoff_MapVal_Vel.png}
        \caption{Accuracy vs. Runtime}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/decoupling/AccuracyVsRuntimeTradeoff_MapVal.png}
        \caption{Accuracy vs. Runtime}
    \end{subfigure}

    \caption{Comprehensive performance comparison of EKF decoupling levels. Each column represents a different feature set: "All Inputs" (left), "Map Val + Vel" (center), and "Map Val" (right). Each row represents a different performance metric: (a-c) Accuracy vs. Complexity, (d-f) Runtime vs. Complexity, and (g-i) Accuracy vs. Runtime trade-off.}
    \label{fig:full_performance_grid}
\end{figure}

\paragraph{Robustness and Consistency Analysis}

The robustness of each decoupling strategy was evaluated by analyzing the statistical distribution of the mean position error over 50 Monte Carlo runs. Figure \ref{fig:full_robustness_grid} shows these distributions for two representative neural network complexities (N=8 and N=48) across the three feature sets.

The results consistently show that the fully-coupled Level 0 EKF is the most robust estimator. In every case, its boxplot is characterized by the lowest median error and a significantly tighter error distribution (smaller interquartile range), indicating reliable and repeatable performance across different noise realizations.

The decoupled filters, in contrast, exhibit significantly more variance. This is particularly dramatic in the "All Inputs, N=8" case, where the distributions for Level 1 and Level 2 are extremely wide, with outliers indicating instances of filter divergence. In contrast, Level 0 remains stable and precise. Even in the converged case ("Map Val + Vel, N=48"), Level 0's box is noticeably smaller and lower than the others. This demonstrates that the mathematical approximations inherent in the decoupling strategies not only increase the average error but also fundamentally reduce the filter's reliability.

% --- FIGURE 2: 2x3 Robustness Grid ---
\begin{figure}[p]
    \centering
    \makebox[0.32\textwidth]{\textbf{All Inputs}} \hfill
    \makebox[0.32\textwidth]{\textbf{Map Val + Vel}} \hfill
    \makebox[0.32\textwidth]{\textbf{Map Val}}
    \vspace{0.2cm}
    
    % --- Row 1: N=8 Neurons ---
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/decoupling/RobustnessComparison_AllInputs_N8.png}
        \caption{N=8 Neurons}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/decoupling/RobustnessComparison_MapVal_Vel_N8.png}
        \caption{N=8 Neurons}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/decoupling/RobustnessComparison_MapVal_N8.png}
        \caption{N=8 Neurons}
    \end{subfigure}
    \vspace{0.5cm}
    
    % --- Row 2: N=48 Neurons ---
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/decoupling/RobustnessComparison_AllInputs_N48.png}
        \caption{N=48 Neurons}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/decoupling/RobustnessComparison_MapVal_Vel_N48.png}
        \caption{N=48 Neurons}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/decoupling/RobustnessComparison_MapVal_N48.png}
        \caption{N=48 Neurons}
    \end{subfigure}
    
    \caption{Robustness comparison of EKF decoupling levels over 50 Monte Carlo runs. Each column represents a different feature set, and each row represents a different neural network complexity (N=8 and N=48). The box plots show the distribution of the mean position error.}
    \label{fig:full_robustness_grid}
\end{figure}


\paragraph{Discussion including CRLB}

The experimental investigation revealed that the standard, fully-coupled EKF configuration was demonstrably superior to the decoupled approximations for the intended application. A key finding emerged from the runtime analysis: the theoretical computational benefits of decoupling were only realized for high-complexity neural network models. For simpler models, the software overhead associated with the fragmented update logic in a high-level environment resulted in slower performance than the highly optimized, consolidated operations of the fully-coupled filter. This created a practical paradox where the optimization was only effective for models likely too complex for a resource-constrained avionics system. 

\subsubsection*{Proposed Design Methodology for an Aircraft Implementation}

Based on the insights from the simulation, we propose a systematic, three-stage methodology for designing an operational EKF-NN for a real-world aircraft. This hierarchical approach deconstructs the complex tuning problem into a sequence of manageable steps, ensuring that foundational decisions inform subsequent optimizations.

\begin{enumerate}
    \item \textbf{Feature Selection.} The initial and most critical stage is to identify the most informative, yet parsimonious, feature set. Using a fixed, high-fidelity filter (i.e., a fully coupled EKF) and a moderately sized neural network, different subsets of available sensor data (e.g., attitude, velocity, air data) are evaluated. The objective is to determine the minimal set of features that captures the majority of the observable magnetic noise dynamics, establishing a robust foundation for the model.

    \item \textbf{Model Sizing.} With the optimal feature set identified, the second stage focuses on tuning the network's complexity. Here, the number of hidden neurons ($N_{\text{hidden}}$) is swept to find the ideal trade-off between the model's approximation capability and its computational footprint. The goal is to find the "knee of the curve," where adding more neurons yields diminishing returns on accuracy at the cost of increased runtime.

    \item \textbf{Computational Optimization.} In the final stage, with the feature set and network architecture now fixed, the EKF's computational structure is optimized. The different decoupling levels are tested to generate a clear Pareto front of estimation accuracy versus runtime. This allows a system designer to select the most efficient implementation (e.g., a block-diagonal or fully diagonal covariance) that meets the strict real-time processing constraints of the target avionics hardware.
\end{enumerate}

This structured process systematically navigates the large design space, ensuring a final configuration that is not only accurate but also robust and computationally feasible for in-flight operation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% END DECOUPLING %%%%%%%%%

The principles demonstrated in this 2D toy model provide a direct conceptual foundation for tackling more complex, real-world estimation problems. The next chapter will address the 3D global navigation of an aircraft using magnetic field measurements, a scenario which shares the same fundamental structure but with increased complexity.

\subsubsection{Discussion}
The investigation into EKF decoupling strategies yielded a critical insight into the trade-offs between theoretical optimization and practical implementation for real-time systems. While the decoupled filters were designed to reduce computational load, our results demonstrate that these runtime benefits only manifest for neural network models of high complexity (i.e., those with a large number of hidden neurons). This presents a practical dilemma, as such complex models may be undesirable for the target application on an aircraft, where simplicity, predictability, and ease of verification are paramount. For the simpler, more suitable models, the standard, fully-coupled EKF was paradoxically found to be superior in all metrics, exhibiting both higher accuracy and lower runtimes. This outcome highlights a key engineering lesson: the software overhead associated with the more fragmented logic of the decoupled updates in a high-level environment can outweigh the theoretical reduction in floating-point operations for problems of low to moderate dimensionality. Therefore, for a resource-constrained application requiring a reasonably simple model, the direct, un-optimized but efficiently implemented fully-coupled EKF represents the optimal engineering choice.

==> notation.tex <==
\begin{table}[hbt!]
\begin{center}
\caption{\label{tab:variables}Notation}
    \begin{tabularx}{\columnwidth}{c|X}
        \toprule \bfseries
        Symbol & \bfseries Description \\ 
        \midrule
        %\hline
        \{n\}, \{e\}, \{d\} & NED coordinate subscripts (north, east, down)  \\   
        \midrule
        $\bm p$, $\bm v$, $\bm \epsilon$ & Position, velocity, and attitude\\
        $\mu, \lambda, \xi$ & Latitude, longitude, and altitude \\
        $\phi$, $\theta$, $\psi$ & Roll, pitch, and yaw angles $\phi, \theta, \psi \in (-\pi, \pi]$ \\
        \midrule
        $\bm{S}(\cdot)$ & Skew symmetric matrix \\
        $\bm{R}_{nb}$ & Attitude / rotation matrix from body to NED \\
        $R_0$ & Equatorial radius $R_0 = \SI{6378137.0}{\meter}$
        \\
        $\omega_{ie}$ & Earth's rotation rate $\omega_{ie} = \SI{7.292115e-5 }{\radian\per\second}$\\
        $\bfg^e$ & Gravitational acceleration in ECEF frame
        \\
        \midrule
        $\bff^b_m$, $\boomega^b_m$ & Specific force and angular rate measurements in body frame \\
        $\bff^b_{ib}$, $\boomega^b_{ib}$ & True specific force and angular velocity \\
        $\boeta_{\boomega}$, $\boeta_{\bfa}$ & Angular rate and acceleration measurement noise \\
        $\bfa_{\bfb}$, $\boomega_{\bfb}$ & Accelerometer and gyroscope biases\\     
        \midrule
        $\delta \bm p$, $\delta \bm v$, $\delta \bm \epsilon$ &  Position, velocity and attitude errors \\
        $\bm x$ & State vector including navigation error states and model parameters\\     
        \midrule
        $\delta \hbfp, \delta \hbfv, \delta \hat{ \bm \epsilon}, \delta \hbfx, ...$ & Estimated quantities\\
        \midrule
        \multicolumn{2}{c}{\bfseries Neural Network Training} \\
        \midrule
        $\bfx_{nn}$ & State vector of neural network parameters (weights and biases) \\
        $\bophi$ & Input feature vector to the neural network \\
        $\bfz$ & Target output vector / ground truth measurement \\
        $\bfh(\cdot)$ & Neural network output function / measurement prediction \\
        $L$ & Mean Squared Error (MSE) loss function \\
        $\eta$ & Learning rate in backpropagation \\
        $\alpha$ & Momentum coefficient in backpropagation \\
        \midrule
        \multicolumn{2}{c}{\bfseries Extended Kalman Filter (EKF)} \\
        \midrule
        $\covP$ & State estimate covariance matrix \\
        $\covQ$ & Process noise covariance matrix ($\covQ_c$ continuous, $\covQ_d$ discrete) \\
        $\covR$ & Measurement noise covariance matrix \\
        $\bfv, \bfw$ & Zero-mean process and measurement noise vectors \\
        $\bfK$ & Kalman gain \\
        $\bfH$ & Jacobian of the measurement function $\bm{h}$ w.r.t. the state \\
        \bottomrule
    \end{tabularx}
\end{center}
%\vspace{-0.8cm}
\end{table}

==> theory.tex <==
\section{A Unified Framework for State Estimation and Model Learning}
%\section{A Unified Perspective on Backpropagation and Kalman Filter Training}
%\section{Unifying Gradients and Recursive Estimation}
%\section{Neural Network Training as a State Estimation Problem}
%\section{Recursive Learning for Simultaneous Navigation and System Identification}
%\section{Foundations of Hybrid EKF-NN Systems for Online Calibration}
\label{sec:theory}

Hybrid \ac{EKF}-\ac{NN} systems are promising for navigation, as the methods' strengths are complementary. \ac{EKF} performance degrades with model inaccuracies or unknown noise (i.e., linearization errors, map inaccuracies, or calibration errors), whereas \ac{NN}s can learn complex, non-linear noise dynamics from data without prior models. This combination leverages the \ac{EKF} efficiency with \ac{NN} data-driven robustness for refining calibration.

NNs are typically integrated with \ac{EKF}s by either performing specific tasks, like predicting \ac{INS} errors during \ac{GNSS} outages to correct state estimates \cite{wang_neural_2007, guo_neural_2013}, or by adaptively tuning the filter's parameters, such as its noise covariance matrices or the Kalman Gain \cite{jouaber_nnakf_2021, revach_kalmannet_2022, Cuenca2024, cohen_inertial_2024}.

A powerful integration strategy augments the \ac{EKF} state vector with the \ac{NN}'s parameters (weights and biases), enabling their continuous, real-time adaptation. The \ac{EKF} updates the \ac{NN} to model unknown non-linear dynamics or noise simultaneously to system state estimation without extensive prior knowledge. The filter's recursive update mechanism itself trains the network, a process analogous to backpropagation. This recursive training inherently encodes temporal information, removing the need to manually add features like measurement derivatives.


%
\subsection{Extended Kalman Filter for Training Neural Networks}
The training of a neural network involves optimizing its weights and biases, a task predominantly accomplished through gradient descent-based algorithms. The most ubiquitous of these is the backpropagation algorithm \cite{Rumelhart1986, Schmidhuber2015}. An alternative paradigm employs recursive estimation techniques, such as the Kalman filter \cite[Ch.~4.2]{BrownHwang2012}, which frames the training process as an optimal state estimation problem. Although conceptually distinct, these two methods are fundamentally linked. It has been demonstrated that the standard backpropagation algorithm can be derived as a limiting case of the \ac{EKF} algorithm when applied to neural network training \cite{ruck_comparative_1992, sarat_chandran_comments_1994}.

To formalize this relationship, we will briefly recap the mathematical basis of backpropagation. As notation conventions often differ between the machine learning and Kalman filtering literature, we will adopt a notation that aligns closely with Kalman filtering to ensure consistency.

Before training begins, standard pre-processing steps are assumed. The input features $\bophi$ and target outputs $\mathbf{z}$ are typically scaled to have zero mean and unit variance to ensure numerical stability and improve convergence. Furthermore, the initial network parameters $\bfx_{NN,0}$ are initialized with small random values drawn from a suitable distribution (e.g., Glorot or He initialization) to break symmetry and prevent issues with vanishing or exploding gradients.

Let $\bfh(\bfx_{NN}, \bophi)$ represent the network's output vector for a given set of parameters (weights and biases) $\bfx_{NN}$ and input features $\bophi$. The corresponding ground truth or target vector is denoted by $\bfz$. For notational simplicity in the following equations, the dependency on input features $\bophi$ will be implicit, and the network output will be written as $\bfh(\bfx_{NN})$.

In classical regression, the goal is to minimize a loss function, typically the \ac{MSE}. For a single training sample, the loss L is given by:
%
\begin{align}
L = \frac{1}{2} (\bfz - \bfh(\bfx_{NN}))^\top(\bfz - \bfh(\bfx_{NN}))
\end{align}
%
The training process is iterative. Denoting the parameter vector at training step t as $\bfx_{NN}(t)$, a common enhancement to the standard update is the inclusion of a momentum term:
%
\begin{align}
\Delta \bfx_{NN} (t) = -\eta \frac{\partial L(t)}{\partial\bfx_{NN}} + \alpha \Delta \bfx_{NN}(t-1)
\end{align}
%
Here, $\boeta$ is the learning rate, and the momentum coefficient $\alpha$ incorporates a fraction of the previous update vector into the current step. This term acts as a form of \enquote(inertia), helping to accelerate convergence along shallow gradients and dampen oscillations in directions of high curvature. This use of historical information to inform the current update is conceptually analogous to the Kalman filter's approach; both methods introduce dynamic memory into the estimation process rather than relying solely on the instantaneous measurement or gradient.

However, to simplify the following comparison and isolate the fundamental mathematical relationship between the two algorithms, we will neglect the momentum term (i.e., set $\alpha=0$) and proceed with the standard gradient descent rule. The update is therefore given by the negative gradient of the loss function:
%
\begin{align}
\Delta \bfx_{NN} (t) &= -\eta \frac{\partial L(t)}{\partial\bfx_{NN}} \nonumber \\
&= \eta \left( \frac{\partial \bfh(\bfx_{NN})}{\partial \bfx_{NN}} \right)^\top (\bfz - \bfh(\bfx_{NN})) \label{eq:delta_weights_nn}
\end{align}
%
We now frame the network training process using an \ac{EKF}. In this paradigm, the network's parameters $\bfx_{NN}$ are treated as the filter's state vector. The weight matrices $\bfW$ and bias vectors $\bfb$ of a network with $L$ layers are flattened into the column vector
 \begin{align}
    \bfx_{NN} = \left[ 
    \text{vec}(\mathbf{W}^{(1)}), 
    \mathbf{b}^{(1)}, 
    \dots, 
    \text{vec}(\mathbf{W}^{(L)}), 
    \mathbf{b}^{(L)} 
 \right]^\top.
 \end{align}
%The evolution of a \ac{EKF} state is described by the general discrete-time linear model 
%\begin{equation}
%    \bfx_t = \bfF \bfx_{t-1} + \bfG \bfu_{t-1} + \bfw_{t-1}
%    \label{eq:ekf_model_dynamics}
%\end{equation}
Ideally, the optimal parameters are time-invariant, suggesting a static process $\dot{\bfx}_{NN} = 0$.
However, a purely static model is problematic. As the filter processes data, its confidence in the parameter estimates would increase, causing the state covariance matrix $\covP$ to shrink. This leads to a vanishing Kalman gain $\bfK$, effectively stopping the learning process. To prevent this and ensure the filter remains adaptive to new information, artificial process noise $\dot{\bfx}(t) = \bfC(t) \bfw(t)$ is introduced to drive the adaptation of the parameters. Assuming for simplicity that the Gaussian noise is applied directly to the states (i.e., $\bfC(t) = \bfI$), the continuous-time process model becomes:
%
\begin{align}
\dot{\bfx}_{NN}(t) &= \bfw(t), \quad \text{where } \bfw(t) \sim \mathcal{N}(0, \bosigma_w^2)
\end{align}
%
The measurement model uses the network's output as the predicted measurement. The relationship between the true output $\bfz(t)$ and the network's prediction $\bfh(\bfx_{NN}(t))$ is given by:
%
\begin{align}
\bfz_t = \bfh(\bfx_{NN,t}) + \bfv_t, \quad \text{where } \bfv_t \sim \mathcal{N}(0, \bosigma_v^2)
\end{align}
%
with the measurement noise spectral density $\covR:= \bosigma_v^2 $. Since the EKF is implemented in discrete time steps, the continuous process noise spectral density $\covQ_c := \bosigma_w^2$ is discretized into $\covQ_d$. This can be done using a simple first-order Euler approximation ($\covQ_d \approx \covQ_c \Delta t$) or through more advanced discretization methods that provide higher accuracy.

The EKF training process then consists of the standard prediction-correction loop. For a static model with added noise, the steps are:

\begin{enumerate}
    \item Prediction (Time Update):
%
    \begin{align}
    \bfx_{t|t-1} &\leftarrow \bfx_{t-1} \\
    \covP_{t|t-1} &\leftarrow \covP_{t-1} + \covQ_d
    \end{align}
    %
    \item Correction (Measurement Update):
    %
    \begin{subequations}
    \begin{align}
    %\nu_t &= \bfz_t - \bfh(\bfx_{NN,t|t-1}) \\
    \bfK_t &= \covP_{t|t-1} \bfH^\top (\bfH \covP_{t|t-1} \bfH^\top + \covR)^{-1} \\
    \bfx_{t} &= \bfx_{t|t-1} + \bfK_t (\bfz_t - \bfh(\bfx_{t|t-1})) \label{eq:kf_update_state} \\
    \covP_t &= (\bfI - \bfK_t \bfH) \covP_{t|t-1} \label{eq:ekf_update_covariance}
    \end{align}
    \label{eq:ekf_update}
    \end{subequations}
\end{enumerate}

%
where $\bfH$ is the Jacobian of the network output $\bfh$ with respect to the parameters $\bfx_{NN}$, evaluated at the current state estimate $\hbfx_NN$.

The update to the network parameters from \cref{eq:kf_update_state} is therefore $\Delta \bfx_{NN,t|t-1} = \bfK_t (\mathbf{z}_t - \mathbf{h}(\bfx_{NN, t|t-1}))$. This expression can be shown to be equivalent to the backpropagation update rule in \cref{eq:delta_weights_nn} under a set of simplifying assumptions. Specifically, if the measurement noise is isotropic ($\covR = \epsilon^{-1}\mathbf{I}$) and the parameter covariance is also isotropic ($\covP = p\mathbf{I}$), the Kalman gain matrix $\bfK$ simplifies to a term proportional to the gradient. This equivalence defines the backpropagation learning rate $\eta$ in terms of the filter's covariance parameters: $\eta = \epsilon^{-1} p$.

\subsection{Tuning}
\label{ssec:tuning_theory}
An consequence of this relationship is that the effective learning rate is distributed among the interdependent covariance matrices: the measurement noise $\covR$, the state covariance $\covP$, and the process noise $\covQ$. Because the underlying process model for the parameters is static, the EKF's behavior is governed by the ratios of these matrices rather than their absolute values. This implies that for any tuning task, one of the three parameters can be held constant, leaving only the other two to be optimized for a given problem \cite[Ch.~2.3.3]{haykin_kalman_2001}.

This connection historically led to the view that EKF training was a fundamentally more powerful alternative to backpropagation. While standard gradient descent is a first-order optimization method (using only the gradient $\nabla L$), the EKF implicitly uses second-order information through the update of its covariance matrix $\covP$. This becomes most apparent when the covariance update \cref{eq:ekf_update_covariance} is formulated in terms of the inverse of the covariance, known as the information or precision matrix $\covP^{-1}$:
%
\begin{align}
    \covP^{-1}_t = \covP^{-1}_{t|t-1} + \mathbf{H}^\top \covR^{-1} \mathbf{H} \label{eq:information_update}
\end{align}
%
For Gaussian distributions, the information matrix is equivalent to the Hessian of the negative log-probability. In this light, \cref{eq:information_update} can be interpreted as a Bayesian update of second-order information. The term $\covP^{-1}_{t|t-1}$ represents the Hessian of the prior parameter distribution, while the term $\mathbf{H}^\top \covR^{-1} \mathbf{H}$ is an approximation of the Hessian related to the new measurement.

However, this historical perspective requires context. The comparison holds true for the simplest form of backpropagation, but the algorithm has evolved significantly. Modern deep learning employs advanced adaptive optimizers like Adam, RMSprop, and AdaGrad. These optimizers, much like the EKF, approximate second-order information to accelerate training by computing an individual, adaptive learning rate for every network parameter.

With this, we've established the important relation between EKF training and standard backpropagation. They are equivalent only when the second-order information, encoded in the covariance update of the Kalman filter, is discarded. While the EKF provides a powerful theoretical framework, modern backpropagation-based methods have developed more scalable techniques to incorporate similar principles, making them the standard for training deep neural networks today.

Despite its computational complexity compared to modern optimizers (scaling quadratically or cubically with the number of parameters), EKF-based training remains valuable in specific domains. The primary advantage of the EKF is its ability to provide a principled estimate of the uncertainty in the network's parameters via the covariance matrix $\covP$. This is critical in applications where the model's confidence in its predictions is as important as the predictions themselves. Consequently, EKF training finds its niche in real-time adaptive systems, particularly with smaller networks where the computational cost is manageable. Key application areas include adaptive control and robotics, where neural networks learn system dynamics online and uncertainty estimates are vital for ensuring safety and stability \cite{puskorius_neurocontrol_1994}, and online system identification, where the filter's sequential nature is ideal for tracking time-varying systems \cite{singhal_training_1988}. To mitigate the computational burden for larger networks, approximation techniques have been developed, such as assuming a block-diagonal structure for the covariance matrix, which significantly improves scalability by ignoring correlations between weights in different layers \cite[Chapter~2]{haykin_kalman_2001}. In these contexts, the superior convergence speed (in terms of epochs) and the rich information provided by the covariance matrix can justify the higher computational cost per training step.

\subsection{Application to Simultaneous Navigation and Model Calibration} 
This theoretical framework enables our application: the online calibration of a magnetic noise model for aircraft magnetic anomaly navigation. We augment the standard \ac{EKF} state vector, comprising navigation and magnetic map states, with the neural network parameters, $\bfx_{NN}$, that model the platform's magnetic interference.

This unified structure is key to online learning. The \ac{NN} becomes an integral part of the filter's measurement equation, predicting the complex magnetic interference generated by aircraft systems. During the \ac{EKF}'s correction step, the magnetic innovation (the difference between measured and predicted fields) is used to update the entire augmented state simultaneously.

Consequently, each magnetometer reading concurrently corrects the aircraft's navigation solution and refines the \ac{NN}'s parameters. This creates a symbiotic process: a more accurate noise model improves navigation, while a better navigation solution provides a cleaner signal for model training. We will demonstrate this simultaneous navigation and system identification approach in the following chapter in a simple model of magnetometer-aided 2D-odometry.
